a-DCF: an architecture agnostic metric with application to spoofing-robust speaker verification

Spoofing detection is today a mainstream research topic. Standard metrics can be applied to evaluate the performance of isolated spoofing detection solutions and others have been proposed to support their evaluation when they are combined with speaker detection. These either have well-known deficiencies or restrict the architectural approach to combine speaker and spoof detectors. In this paper, we propose an architecture-agnostic detection cost function (a-DCF). A generalisation of the original DCF used widely for the assessment of automatic speaker verification (ASV), the a-DCF is designed for the evaluation of spoofing-robust ASV. Like the DCF, the a-DCF reflects the cost of decisions in a Bayes risk sense, with explicitly defined class priors and detection cost model. We demonstrate the merit of the a-DCF through the benchmarking evaluation of architecturally-heterogeneous spoofing-robust ASV solutions.

==> tables/cost_definition.tex <==
\begin{table}[]
\caption{Costs for evaluating the SASV system. If bonafide speech is rejected by the SASV system, it is counted as miss rates(). The opposite error cases include nontarget speech or spoof speech is accepted as false acceptance ()}
  \centering
  \label{tab:cost_def}
    \begin{tabular}{|l|l|l|l|}
    \hline
     & Target_{True} & NonTar_{True} & Spoof_{True} \\ \hline
    Target_{Sys} & 0 & C^{\text{non}}_{fa} & C^{\text{spf}}_{fa} \\
    NonTar_{Sys} & C^{\text{tar}}_{miss} & 0 & 0 \\
    Spoof_{Sys} & C^{\text{tar}}_{miss} & 0 & 0 \\ \hline
    \end{tabular}
\end{table}

==> tables/single_adcf.tex <==
\begin{table*}[t]
  \caption{
  a-DCF results of single integrated systems.
  Eight different systems from Mun et. al.~\cite{mun2023towards} have been evaluated with the EERs adopted in SASV challenge 2022 and the proposed $a$-DCF with four different DCF priors.}
  \centering
  \label{tab:single_result}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|ccc|cccc|cccc|}
    \hline
     &  & EERs &  & \multicolumn{4}{c|}{(Normalized) min a-DCFs} & \multicolumn{4}{c|}{Thresholds} \\
    \multicolumn{1}{|c|}{} & SASV-EER & SV-EER & SPF-EER & a-DCF1 & a-DCF2 & a-DCF3 & a-DCF4 & a-DCF1 & a-DCF2 & a-DCF3 & a-DCF4 \\ \hline
    \multicolumn{1}{|c|}{S1} & 1.19 & 1.82 & 0.58 & 0.0276 & 0.0406 & 0.0222 & 0.0578 & 0.5221 & 0.5221 & 0.4654 & 0.4654 \\
    \multicolumn{1}{|c|}{S2} & 1.25 & 1.27 & 1.23 & 0.0262 & 0.0301 & 0.0268 & 0.0417 & 0.5323 & 0.5022 & 0.4867 & 0.4668 \\
    \multicolumn{1}{|c|}{S3} & 1.82 & 2.51 & 1.16 & 0.0426 & 0.0594 & 0.0366 & 0.0853 & 0.5100 & 0.4952 & 0.4512 & 0.4437 \\
    \multicolumn{1}{|c|}{S4} & 2.48 & 3.32 & 1.56 & 0.0571 & 0.0781 & 0.0485 & 0.1068 & 0.5365 & 0.5365 & 0.5005 & 0.4585 \\
    \multicolumn{1}{|c|}{S5} & 5.94 & 10.20 & 1.99 & 0.1492 & 0.22318 & 0.0965 & 0.2544 & 0.5136 & 0.5136 & 0.4105 & 0.3932 \\
    \multicolumn{1}{|c|}{S6} & 9.55 & 15.14 & 5.06 & 0.2318 & 0.3373 & 0.1759 & 0.3962 & 0.5645 & 0.5601 & 0.4473 & 0.3865 \\
    \multicolumn{1}{|c|}{S7} & 9.57 & 14.41 & 5.56 & 0.2296 & 0.3341 & 0.1882 & 0.4288 & 0.5858 & 0.5681 & 0.4865 & 0.4183 \\
    \multicolumn{1}{|c|}{S8} & 11.47 & 13.46 & 10.30 & 0.2495 & 0.3256 & 0.2709 & 0.4759 & 0.5350 & 0.4895 & 0.4826 & 0.3621 \\ \hline
\end{tabular}
}
\end{table*}

==> tables/single_adcf2.tex <==
\begin{table*}[t]
  \caption{
  EERs and a-DCF results of diverse categories of systems.
  Four different single-model systems are from \cite{mun2023towards} (S1-S4). Three systems are from SASV challenge 2022 (C1-C3), One system from \autoref{tab:tandem_adcf} (C4).
  Best performing system for each ``S'' and ``C'' are boldfaced.}
  \centering
  \label{tab:single_result}
  \begin{tabular}{l|l|ccc|cccc|c}
  \toprule
 & \multirow{2}{*}{\textbf{System type}} & \multicolumn{3}{c|}{\textbf{EERs}} & \multicolumn{4}{c}{\textbf{min a-DCF}s}  \\
 &  & \textbf{SASV-EER} & \textbf{SV-EER} & \textbf{SPF-EER} & \textbf{a-DCF1} & \textbf{a-DCF2} & \textbf{a-DCF3} & \textbf{a-DCF4} & \textbf{t-DCF}\\
 \toprule
 S1 & Single-model & \textbf{1.19} & 1.82 & \textbf{0.58} & 0.0276 & 0.0406 & \textbf{0.0222} & 0.0578 \\
S2 & Single-model & 1.25 & \textbf{1.27} & 1.23 & \textbf{0.0262} & \textbf{0.0301} & 0.0268 & \textbf{0.0417} \\
S3 & Single-model & 1.82 & 2.51 & 1.16 & 0.0426 & 0.0594 & 0.0366 & 0.0853 \\
S4 & Single-model & 2.48 & 3.32 & 1.56 & 0.0571 & 0.0781 & 0.0485 & 0.1068 \\
\hline
C1 & Jointly optimized (\em \small score) & \textbf{0.13} & \textbf{0.11} & \textbf{0.17} & \textbf{0.0025} & \textbf{0.0026} & \textbf{0.0032} & \textbf{0.0060} \\
C2 & Jointly optimized ({\em \small embedding}) & 0.28 & 0.28 & 0.28 & 0.0058 & 0.0070 & 0.0067 & 0.0147 \\
C3 & Jointly optimized (\em \small score) & 0.37 & 0.45 & 0.26 & 0.0070 & 0.0100 & 0.0080 & 0.0219 \\
C4 & Cascade & 0.76 & 0.71 & 0.80 & 0.0153 & 0.0180 & 0.0180 & 0.0382 \\
\bottomrule
\end{tabular}

\end{table*}


==> tables/single_adcf3.tex <==
\begin{table*}[t]
  \caption{
  EERs and a-DCF results of diverse categories of systems.
  Eight different single-model, ``S,'' systems from \cite{mun2023towards} and six systems that ranked the highest in SASV challenge 2022, ``C,'' have been employed.
  Best performing system for ``S'' and ``C'' are boldfaced respectively.}
  \centering
  \label{tab:single_result}
  %\resizebox{\textwidth}{!}{
  \begin{tabular}{l|l|ccc|cccc}
\toprule
 & \multirow{2}{*}{\textbf{System type}} & \multicolumn{3}{c|}{\textbf{EERs}} & \multicolumn{4}{c}{\textbf{min a-DCF}s} \\ %\cline{3-5}
 &  & \textbf{SASV-EER} & \textbf{SV-EER} & \textbf{SPF-EER} & \textbf{a-DCF1} & \textbf{a-DCF2} & \textbf{a-DCF3} & \textbf{a-DCF4} \\
 \toprule
 S1 & Single-model & \textbf{1.19} & 1.82 & \textbf{0.58} & 0.0276 & 0.0406 & \textbf{0.0222} & 0.0578 \\
 %& N/A\\
S2 & Single-model & 1.25 & \textbf{1.27} & 1.23 & \textbf{0.0262} & \textbf{0.0301} & 0.0268 & \textbf{0.0417} \\
 %& N/A\\
S3 & Single-model & 1.82 & 2.51 & 1.16 & 0.0426 & 0.0594 & 0.0366 & 0.0853 \\
%& N/A\\
S4 & Single-model & 2.48 & 3.32 & 1.56 & 0.0571 & 0.0781 & 0.0485 & 0.1068 \\
%& N/A\\
S5 & Single-model & 5.94 & 10.20 & 1.99 & 0.1492 & 0.2231 & 0.0965 & 0.2544 \\
%& N/A\\
S6 & Single-model & 9.55 & 15.14 & 5.06 & 0.2318 & 0.3373 & 0.1759 & 0.3962 \\
%& N/A\\
S7 & Single-model & 9.57 & 14.41 & 5.56 & 0.2296 & 0.3341 & 0.1882 & 0.4288 \\
%& N/A\\
S8 & Single-model & 11.47 & 13.46 & 10.30 & 0.2495 & 0.3256 & 0.2709 & 0.4759 \\ \hline
%& N/A\\ \hline
C1 & Jointly optimized (\em \small score) & \underline{\textbf{0.13}} & \underline{\textbf{0.11}} & \underline{\textbf{0.17}} & \underline{\textbf{0.0025}} & \underline{\textbf{0.0026}} & \underline{\textbf{0.0032}} & \underline{\textbf{0.0060}} \\
%& N/A\\
C2 & Cascade & 0.21 & 0.46 & 0.19 & 0.0051 & 0.0069 & 0.0046 & 0.0116 \\
%& \\
C3 & Jointly optimized ({\em \small embedding}) & 0.28 & 0.28 & 0.28 & 0.0058 & 0.0070 & 0.0067 & 0.0147 \\
%& N/A\\
C4 & Jointly optimized (\em \small score) & 0.37 & 0.45 & 0.26 & 0.0070 & 0.0100 & 0.0080 & 0.0219 \\
%& N/A\\
C5 & Jointly optimized (\em \small score) & 0.56 & 0.86 & 0.35 & 0.0132 & 0.0187 & 0.0114 & 0.0271 \\
%& N/A\\
C6 & Jointly optimized (\em \small score) & 0.56 & 0.73 & 0.43 & 0.0117 & 0.0167 & 0.0128 & 0.0338 \\
%& N/A\\
\bottomrule
  \end{tabular}
  %}
\end{table*}

==> tables/single_adcf4.tex <==
\begin{table*}[t]
  \caption{
  EERs and a-DCF results of diverse categories of systems.
  Four different single-model systems are from \cite{mun2023towards} (S1-S4). Three systems are from SASV challenge 2022 (C1-C3), One system from \autoref{tab:tandem_adcf} (C4).
  For a-DCF, best performing systems are boldfaced.}
  \centering
  \label{tab:single_result}
  \begin{tabular}{l|l|ccc|cc|c}
  \toprule
 & \multirow{2}{*}{\textbf{System type}} & \multicolumn{3}{c|}{\textbf{EERs}} & \multicolumn{2}{c}{\textbf{min a-DCF}s}  \\
 &  & \textbf{SASV-EER} & \textbf{SV-EER} & \textbf{SPF-EER} &  \textbf{a-DCF1} & \textbf{a-DCF2} & \textbf{t-DCF}\\
 \toprule
 S1 & Single-model & 1.19 & 1.82 & 0.58  & 0.0222 & 0.0578 &N/A\\
S2 & Single-model & 1.25 & 1.27 & 1.23 & 0.0268 & 0.0417 &N/A\\
S3 & Single-model & 1.82 & 2.51 & 1.16 & 0.0366 & 0.0853 &N/A\\
S4 & Single-model & 2.48 & 3.32 & 1.56 & 0.0485 & 0.1068 &N/A\\
\hline
C1 & Jointly optimized (\em \small score) & 0.13 & 0.11 & 0.17 & \textbf{0.0032} & \textbf{0.0060} &N/A\\
C2 & Jointly optimized ({\em \small embedding}) & 0.28 & 0.28 & 0.28 & 0.0067 & 0.0147 &N/A\\
C3 & Jointly optimized (\em \small score) & 0.37 & 0.45 & 0.26 & 0.0080 & 0.0219 &N/A\\
C4 & Cascade & 0.89 & 0.74 & 0.91 & 0.1492 & 0.0506 & 0.0358\\
\bottomrule
\end{tabular}

\end{table*}


==> tables/tandem_adcf.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!th]
\caption{
a-DCF results of cascade (decision-level tandem) systems.
Pretrained RawNet3~\cite{jung2022pushing} is employed as the ASV and AASIST~\cite{jung2022aasist}, AASIST-L, and LCNN~\cite{} models are employed as the CM.
Performances reported with the EERs adopted in SASV challenge 2022 and the proposed $a$-DCF with four different DCF priors.
}
  \centering
  \label{tab:tandem_adcf}
  \resizebox{\textwidth}{!}{
\begin{tabular}{c|l|ccc|cccc|cccc|}
\cline{2-13}
 & \multirow{2}{*}{Cascade system:threshold} & \multirow{2}{*}{SASV-EER} & \multirow{2}{*}{SV-EER} & \multirow{2}{*}{SPF-EER} & \multicolumn{4}{c|}{Min a-DCFs} & \multicolumn{4}{c|}{Thresholds} \\
 &  &  &  &  & a-DCF1 & a-DCF2 & a-DCF3 & a-DCF4 & a-DCF1 & a-DCF2 & a-DCF3 & a-DCF4 \\ \hline
\multicolumn{1}{|c|}{\multirow{6}{*}{rawnet3 + AASIST}} & \quad\quad\quad ASV: 0.05 & 21.51 & 44.45 & 0.6500 & 0.4627 & 0.6895 & 0.1492 & 0.4316 & 1.5867 & 1.5867 & 1.5817 & 0.6365 \\
\multicolumn{1}{|c|}{} & \quad\quad\quad 
 ASV: 0.5 & 0.89 & 0.74 & 0.9100 & 0.0142 & 0.0189 & 0.1492 & 0.0506 & 1.4803 & 0.6363 & 1.5817 & 0.6363 \\
\multicolumn{1}{|c|}{} & \quad\quad\quad 
 ASV: 0.95 & 100.00 & 100.00 & 100.00 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & -inf & -inf & -inf & -inf \\
\multicolumn{1}{|c|}{} & \quad\quad\quad 
 CM: 0.05 & 1.10 & 0.69 & 1.4900 & 0.01915 & 0.01874 & 0.02407 & 0.0405 & 0.4907 & 0.4907 & 0.4743 & 0.4513 \\
\multicolumn{1}{|c|}{} & \quad\quad\quad CM: 0.5 & 0.76 & 0.71 & 0.8000 & 0.0153 & 0.0180 & 0.0180 & 0.0382 & 0.4907 & 0.4907 & 0.4513 & 0.4513 \\
\multicolumn{1}{|c|}{} & \quad\quad\quad CM: 0.95 & 0.73 & 0.80 & 0.4900 & 0.0142 & 0.0194 & 0.0164 & 0.0424 & 0.4907 & 0.4907 & 0.4513 & 0.4513 \\ \hline
\multicolumn{1}{|c|}{\multirow{6}{*}{rawnet3 + AASIST-L}} & \quad\quad\quad ASV: 0.05 & 21.68 & 44.71 & 0.8200 & 0.4664 & 0.6950 & 0.1551 & 0.4405 & 2.0613 & 2.0002 & 1.7388 & 0.7958 \\
\multicolumn{1}{|c|}{} & \quad\quad\quad ASV: 0.5 & 1.02 & 0.74 & 1.0400 & 0.0160 & 0.0207 & 0.0222 & 0.0560 & 1.3233 & 0.2714 & 1.3233 & 0.2714 \\
\multicolumn{1}{|c|}{} & \quad\quad\quad ASV: 0.95 & 100.00 & 100.00 & 100.00 & 1.00 & 1.00 & 1.0000 & 1.0000 & -inf & -inf & -inf & -inf \\
\multicolumn{1}{|c|}{} & \quad\quad\quad CM: 0.05 & 1.58 & 0.69 & 2.2400 & 0.02443 & 0.02056 & 0.03224 & 0.0453 & 0.4907 & 0.4907 & 0.4513 & 0.4513 \\
\multicolumn{1}{|c|}{} & \quad\quad\quad CM: 0.5 & 1.02 & 0.78 & 1.3000 & 0.0193 & 0.0204 & 0.0241 & 0.0448 & 0.4907 & 0.4907 & 0.4513 & 0.4513 \\
\multicolumn{1}{|c|}{} & \quad\quad\quad CM: 0.95 & 0.82 & 0.84 & 0.7300 & 0.0165 & 0.0210 & 0.0198 & 0.0467 & 0.4907 & 0.4907 & 0.4513 & 0.4513 \\ \hline
\multicolumn{1}{|c|}{\multirow{6}{*}{rawnet3 + LCNN}} & \quad\quad\quad ASV: 0.05 & 21.38 & 42.18 & 2.3900 & 0.4723 & 0.6919 & 0.1754 & 0.4541 & 9.7665 & 9.0800 & 8.3958 & 3.7384 \\
\multicolumn{1}{|c|}{} & \quad\quad\quad ASV: 0.5 & 0.89 & 0.74 & 0.9100 & 0.0126 & 0.0180 & 0.0169 & 0.0479 & -0.2698 & -1.3862 & -0.2698 & -1.3862 \\
\multicolumn{1}{|c|}{} & \quad\quad\quad ASV: 0.95 & 100.00 & 100.00 & 100.00 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & -inf & -inf & -inf & -inf \\
\multicolumn{1}{|c|}{} & \quad\quad\quad CM: 0.05 & 0.63 & 0.74 & 0.5200 & 0.01241 & 0.01764 & 0.01434 & 0.0377 & 0.4907 & 0.4907 & 0.4743 & 0.4526 \\
\multicolumn{1}{|c|}{} & \quad\quad\quad CM: 0.5 & 0.63 & 0.74 & 0.5200 & 0.0123 & 0.0176 & 0.0142 & 0.0375 & 0.4907 & 0.4907 & 0.4743 & 0.4526 \\
\multicolumn{1}{|c|}{} & \quad\quad\quad CM: 0.95 & 0.67 & 0.78 & 0.5100 & 0.0126 & 0.0182 & 0.0146 & 0.0392 & 0.4907 & 0.4907 & 0.4743 & 0.4526 \\ \hline
\end{tabular}
}
\end{table*}

==> tables/tandem_adcf2.tex <==
\begin{table*}[!th]
\caption{
Results of cascade (decision-level tandem with an AND gate) systems.
Pretrained RawNet3~\cite{jung2022pushing} is employed as the ASV and AASIST~\cite{jung2022aasist}, AASIST-L, and LCNN~\cite{lavrentyeva2019stc} models are employed as the CM.
EERs adopted in SASV challenge 2022 are reported. 
Proposed $a$-DCF with four different DCF priors is also employed ($a$-DCF3 has the most similar priors with $t$-DCF).
t-DCF is reported with $\pi_{spf}$=$0.05$, where we did not use the predefined ASV from ASVspoof, but used RawNet3 to be consistent with other metrics.
The best performance per ASV and CM combined are boldfaced and the best performance across all rows underlined.
}
  \centering
  \label{tab:tandem_adcf}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{c|l|ccc|cccc|c}
    \hline
     & \multirow{2}{*}{Cascade system: threshold} & %\multirow{2}{*}{SASV-EER} & %\multirow{2}{*}{SV-EER} & %\multirow{2}{*}{SPF-EER} & 
     \multicolumn{3}{c|}{EERs} & 
     \multicolumn{4}{c|}{min a-DCFs} & \multirow{2}{*}{min t-DCF} \\ %\cline{6-9}
     &  & SASV-EER & SV-EER & SPF-EER & a-DCF1 & a-DCF2 & a-DCF3 & a-DCF4 &  \\ \hline
    \multirow{7}{*}{RawNet3 + AASIST} & ASV$\rightarrow$CM ($t_\text{asv}=0.05$) & 21.51 & 44.45 & 0.65 & 0.4627 & 0.6895 & 0.1492 & 0.4316 & 0.0227 \\
     & ASV$\rightarrow$CM ($t_\text{asv}=0.5$) & 0.89 & 0.74 & 0.91 & 0.0142 & 0.0189 & 0.1492 & 0.0506 & 0.0358\\
     & ASV$\rightarrow$CM ($t_\text{asv}=0.7$) & 17.13 & 17.13 & 17.13 & 0.1747 & 0.2717 & 0.2736 & 0.8494 &  0.0524\\
     % & ASV: 0.95 & 100.00 & 100.00 & 100.00 & 1.0000 & 1.0000 & 1.0000 & 1.0000 &  \\ 
     % \cline{2-9}
     & CM$\rightarrow$ASV ($t_\text{cm}=0.05$) & 1.10 & 0.69 & 1.49 & 0.0191 & 0.0187 & 0.0240 & 0.0405 & N/A \\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.5$) & 0.76 & 0.71 & 0.80 & 0.0153 & 0.0180 & 0.0180 & 0.0382 & N/A \\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.95$) & \textbf{0.73} & 0.80 & 0.49 & 0.0142 & 0.0194 & \textbf{0.0164} & 0.0424 & N/A \\ \hline
    \multirow{7}{*}{RawNet3 + AASIST-L} & ASV$\rightarrow$CM ($t_\text{asv}=0.05$) & 21.68 & 44.71 & 0.82 & 0.4664 & 0.6950 & 0.1551 & 0.4405 & 0.0264 \\
     & ASV$\rightarrow$CM ($t_\text{asv}=0.5$) & 1.02 & 0.74 & 1.04 & 0.0160 & 0.0207 & 0.0222 & 0.0560 & 0.0379 \\
     & ASV$\rightarrow$CM ($t_\text{asv}=0.7$) & 17.13 & 17.13 & 17.13 & 0.1757 & 0.2725 & 0.2752 & 0.8519 & 0.0540\\
     % & ASV: 0.95 & 100 & 100 & 100.00 & 1.0000 & 1.0000 & 1.0000 & 1.0000 &  \\ 
     % \cline{2-9}
     & CM$\rightarrow$ASV ($t_\text{cm}=0.05$)& 1.58 & 0.69 & 2.24 & 0.0244 & 0.0205 & 0.0322 & 0.0453 & N/A \\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.5$) & 1.02 & 0.78 & 1.30 & 0.0193 & 0.0204 & 0.0241 & 0.0448 & N/A \\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.95$)& \textbf{0.82} & 0.84 & 0.73 & 0.0165 & 0.0210 & \textbf{0.0198} & 0.0467 & N/A \\ \hline
    \multirow{6}{*}{RawNet3 + LCNN} & ASV$\rightarrow$CM ($t_\text{asv}=0.05$) & 21.38 & 42.18 & 2.39 & 0.4723 & 0.6919 & 0.1754 & 0.4541 & 0.0577 \\
     & ASV$\rightarrow$CM ($t_\text{asv}=0.5$) & 0.89 & 0.74 & 0.91 & 0.0126 & 0.0180 & 0.0169 & 0.0479 &  0.0728\\
     & ASV$\rightarrow$CM ($t_\text{asv}=0.7$) & 17.13 & 17.13 & 17.13 & 0.1732 & 0.2708 & 0.2713 & 0.8471 & 0.0884 \\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.05$) & 0.63 & 0.74 & 0.52 & 0.0124 & 0.0176 & 0.0143 & 0.0377 & N/A \\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.5$) & \underline{\textbf{0.63}} & 0.74 & 0.52 & 0.0123 & 0.0176 & \underline{\textbf{0.0142}} & 0.0375 & N/A \\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.95$) & 0.67 & 0.78 & 0.51 & 0.0126 & 0.0182 & 0.0146 & 0.0392 & N/A \\ \hline
    \end{tabular}
    }
\end{table*}

==> tables/tandem_adcf3.tex <==
\begin{table*}[!th]
\caption{
Results of cascade (decision-level tandem with an AND gate) systems.
Pretrained RawNet3~\cite{jung2022pushing} is employed as the ASV and AASIST~\cite{jung2022aasist}, AASIST-L, and models are employed as the CM.
The three EERs adopted in SASV challenge 2022 are reported. 
Two a-DCF and t-DCF scenarios are reported respectively.
% Proposed $a$-DCF with four different DCF priors is also employed ($a$-DCF3 has the most similar priors with $t$-DCF).
% t-DCF is reported with $\pi_{spf}$=$0.05$, where we did not use the predefined ASV from ASVspoof, but used RawNet3 to be consistent with other metrics.
The best performance per ASV and CM combined are boldfaced and the best performance across all rows underlined.
}
  \centering
  \label{tab:tandem_adcf}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{c|l|ccc|cc|cc}
    \hline
     & \textbf{Cascade system} & 
     \multicolumn{3}{c|}{\textbf{EERs}} & 
     \multicolumn{2}{c|}{\textbf{min a-DCFs}} & \multicolumn{2}{c}{\textbf{min t-DCFs}} \\ %\cline{6-9}
     & (threshold $t$) & \textbf{SASV-EER} & \textbf{SV-EER} & \textbf{SPF-EER} & \textbf{a-DCF3} & \textbf{a-DCF4} & \textbf{t-DCF3} & \textbf{t-DCF4} \\ \hline
    \multirow{4}{*}{RawNet3 + AASIST} & ASV$\rightarrow$CM ($t_\text{asv}=0.05$) & 21.51 & 44.45 & 0.65 
    %& 0.4627 & 0.6895 & 
    & 0.1492 & 0.4316 
    & \underline{\textbf{0.0226}} &  \textbf{0.0644}\\
     & ASV$\rightarrow$CM ($t_\text{asv}=0.5$) & 0.89 & 0.74 & 0.91 
     %& 0.0142 & 0.0189 
     & 0.1492 & 0.0506 
     & 0.0358 & 0.0918\\
     % & ASV$\rightarrow$CM ($t_\text{asv}=0.7$) & 17.13 & 17.13 & 17.13 
     %& 0.1747 & 0.2717 
     % & 0.2736 & 0.8494 
     % &  0.0524 & 0.1326\\
     % & ASV: 0.95 & 100.00 & 100.00 & 100.00 & 1.0000 & 1.0000 & 1.0000 & 1.0000 &  \\ 
     % \cline{2-9}
     & CM$\rightarrow$ASV ($t_\text{cm}=0.05$) & 1.10 & \underline{\textbf{0.69}} & 1.49 
     %& 0.0191 & 0.0187 
     & 0.0240 & 0.0405 
     & N/A & N/A\\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.5$) & 0.76 & 0.71 & 0.80 
     %& 0.0153 & 0.0180 
     & 0.0180 & \textbf{0.0382} 
    & N/A & N/A\\
     % & CM$\rightarrow$ASV ($t_\text{cm}=0.95$) & \textbf{0.73} & 0.80 & \underline{\textbf{0.49}} 
     %& 0.0142 & 0.0194 
     % & \textbf{0.0164} & 0.0424 
    % & N/A & N/A \\ 
    \hline
    \multirow{4}{*}{RawNet3 + AASIST-L} & ASV$\rightarrow$CM ($t_\text{asv}=0.05$) & 21.68 & 44.71 & 0.82 
    %& 0.4664 & 0.6950 
    & 0.1551 & 0.4405 
    & \textbf{0.0264} & \underline{\textbf{0.0633}}\\
     & ASV$\rightarrow$CM ($t_\text{asv}=0.5$) & 1.02 & 0.74 & 1.04 
     %& 0.0160 & 0.0207 
     & 0.0222 & 0.0560 
     & 0.0379 & 0.0883\\
     % & ASV$\rightarrow$CM ($t_\text{asv}=0.7$) & 17.13 & 17.13 & 17.13 
     %& 0.1757 & 0.2725 
     % & 0.2752 & 0.8519 
     % & 0.0540 & 0.1290\\
     % & ASV: 0.95 & 100 & 100 & 100.00 & 1.0000 & 1.0000 & 1.0000 & 1.0000 &  \\ 
     % \cline{2-9}

     & CM$\rightarrow$ASV ($t_\text{cm}=0.05$)& 1.58 & \underline{\textbf{0.69}} & 2.24 
     %& 0.0244 & 0.0205 
     & 0.0322 & 0.0453 
     & N/A & N/A \\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.5$) & 1.02 & 0.78 & 1.30 
     %& 0.0193 & 0.0204 
     & 0.0241 & \textbf{0.0448} 
     & N/A & N/A \\
     % & CM$\rightarrow$ASV ($t_\text{cm}=0.95$)& \textbf{0.82} & 0.84 & \textbf{0.73} 
     %& 0.0165 & 0.0210 
     % & \textbf{0.0198} & 0.0467 
    % & N/A & N/A \\ 
    \hline
    \iffalse
    \multirow{4}{*}{RawNet3 + LCNN} & ASV$\rightarrow$CM ($t_\text{asv}=0.05$) & 21.38 & 42.18 & 2.39 
    %& 0.4723 & 0.6919 
    & 0.1754 & 0.4541 
    & \textbf{0.0577} & \textbf{0.0995} \\
     & ASV$\rightarrow$CM ($t_\text{asv}=0.5$) & 0.89 & \textbf{0.74} & 0.91 
     %& 0.0126 & 0.0180 
     & 0.0169 & 0.0479 
     & 0.0728 & 0.1312\\
     % & ASV$\rightarrow$CM ($t_\text{asv}=0.7$) & 17.13 & 17.13 & 17.13 
     %& 0.1732 & 0.2708 
     % & 0.2713 & 0.8471 
     % & 0.0884 & 0.1704\\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.05$) & 0.63 & \textbf{0.74} & 0.52 
     %& 0.0124 & 0.0176 
     & 0.0143 & 0.0377 
     & N/A & N/A\\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.5$) & \underline{\textbf{0.63}} & \textbf{0.74} & 0.52 
     %& 0.0123 & 0.0176 & 
     & \underline{\textbf{0.0142}} & \underline{\textbf{0.0375}} 
     & N/A & N/A\\
     % & CM$\rightarrow$ASV ($t_\text{cm}=0.95$) & 0.67 & 0.78 & \textbf{0.51} 
     %& 0.0126 & 0.0182 
     % & 0.0146 & 0.0392 
     % & N/A & N/A\\ 
     \fi
     \hline
    \end{tabular}
    }
\end{table*}

==> tables/tandem_adcf4.tex <==
\begin{table*}[b]
\caption{
Results of cascade (decision-level tandem with an AND gate) systems.
Pretrained RawNet3~\cite{jung2022pushing} is employed as the ASV and AASIST~\cite{jung2022aasist}, AASIST-L, and LCNN~\cite{lavrentyeva2019stc} models are employed as the CM.
EERs adopted in SASV challenge 2022 are reported. 
Proposed $a$-DCF with four different DCF priors is also employed ($a$-DCF3 has the most similar priors with $t$-DCF).
The best performance per a threshold are marked by boldfaced.
}
  \centering
  \label{tab:tandem_adcf}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{c|l|ccc|cc|cc}
    \toprule
     \textbf{System} &
     \textbf{Cascade system} & 
     \multicolumn{3}{c|}{\textbf{EERs}} & 
     \multicolumn{2}{c|}{\textbf{min a-DCFs}} & \multicolumn{2}{c}{\textbf{min t-DCFs}} \\ %\cline{6-9}
     (threshold $t$) & & \textbf{SASV-EER} & \textbf{SV-EER} & \textbf{SPF-EER} & \textbf{a-DCF3} & \textbf{a-DCF4} & \textbf{t-DCF3} & \textbf{t-DCF4} \\ \toprule
    \multirow{3}{*} {ASV$\rightarrow$CM ($t_\text{asv}=0.05$)} & {RawNet3 + AASIST} & 21.51 & 44.45 & \textbf{0.65} & \textbf{0.1492} & \textbf{0.4316} 
    & \textbf{0.0226} &  0.0644\\
    & {RawNet3 + AASIST-L} & 21.68 & 44.71 & 0.82 & 0.1551 & 0.4405 & 0.0264 & \textbf{0.0633}\\
    & {RawNet3 + LCNN} & \textbf{21.38} & \textbf{42.18} & 2.39 & 0.1754 & 0.4541 & 0.0577 & 0.0995 \\
    \hline
    \multirow{3}{*} {ASV$\rightarrow$CM ($t_\text{asv}=0.5$)} & {RawNet3 + AASIST}  & \textbf{0.89} & \textbf{0.74} & \textbf{0.91} & 0.1492 & 0.0506  & \textbf{0.0358} & 0.0918\\
    & {RawNet3 + AASIST-L} & 1.02 & \textbf{0.74} & 1.04 & \textbf{0.0222} & \textbf{0.0560} & 0.0379 & \textbf{0.0883}\\
    & {RawNet3 + LCNN} & \textbf{0.89} & \textbf{0.74} & \textbf{0.91} & 0.0169 & 0.0479 & 0.0728 & 0.1312\\
    % \hline
    % \multirow{3}{*} {ASV$\rightarrow$CM ($t_\text{asv}=0.7$)} & {RawNet3 + AASIST} & \textbf{17.13} & \textbf{17.13} & \textbf{17.13} & 0.2736 & 0.8494 &  \textbf{0.0524} & 0.1326\\
    % & RawNet3 + AASIST-L & \textbf{17.13} & \textbf{17.13} & \textbf{17.13} & 0.2752 & 0.8519 & 0.0540 & \textbf{0.1290}\\
    % & RawNet3 + LCNN & \textbf{17.13} & \textbf{17.13} & \textbf{17.13} & \textbf{0.2713} & \textbf{0.8471} & 0.0884 & 0.1704\\
    \hline \hline
    \multirow{3}{*} {CM$\rightarrow$ASV ($t_\text{cm}=0.05$)} & {RawNet3 + AASIST} & 1.10 & \textbf{0.69} & 1.49 & 0.0240 & 0.0405 & N/A & N/A\\
    & RawNet3 + AASIST-L & 1.58 & \textbf{0.69} & 2.24 & 0.0322 & 0.0453 & N/A & N/A \\
    & RawNet3 + LCNN & \textbf{0.63} & 0.74 & \textbf{0.52} & \textbf{0.0143} & \textbf{0.0377} & N/A & N/A\\
    \hline
    \multirow{3}{*} {CM$\rightarrow$ASV ($t_\text{cm}=0.5$)} & {RawNet3 + AASIST} & 0.76 & \textbf{0.71} & 0.80 & 0.0180 & 0.0382 & N/A & N/A\\
    & RawNet3 + AASIST-L & 1.02 & 0.78 & 1.30 & 0.0241 & 0.0448 & N/A & N/A \\
    & RawNet3 + LCNN & \textbf{0.63} & 0.74 & \textbf{0.52} & \textbf{0.0142} & \textbf{0.0375} & N/A & N/A\\
    % \hline
    % \multirow{3}{*} {CM$\rightarrow$ASV ($t_\text{cm}=0.95$)} & {RawNet3 + AASIST} & 0.73 & 0.80 & \textbf{0.4} & 0.0164 & 0.0424 & N/A & N/A\\
    % & RawNet3 + AASIST-L & 0.82 & 0.84 & 0.73 & 0.0198 & 0.0467 & N/A & N/A\\
    % & RawNet3 + LCNN & \textbf{0.67} & \textbf{0.78} & 0.51 & \textbf{0.0146} & \textbf{0.0392} & N/A & N/A\\
    \bottomrule
    \end{tabular}
    }
\end{table*}

==> tables/tandem_adcf5.tex <==
\begin{table*}[!th]
\caption{
Results of cascade (decision-level tandem with an AND gate) systems.
Pretrained RawNet3~\cite{jung2022pushing} is employed as the ASV and AASIST~\cite{jung2022aasist}, AASIST-L, and models are employed as the CM.
The three EERs adopted in SASV challenge 2022 are reported. 
Two a-DCF and t-DCF scenarios are reported respectively.
% Proposed $a$-DCF with four different DCF priors is also employed ($a$-DCF3 has the most similar priors with $t$-DCF).
% t-DCF is reported with $\pi_{spf}$=$0.05$, where we did not use the predefined ASV from ASVspoof, but used RawNet3 to be consistent with other metrics.
%The best performance per ASV and CM combined are boldfaced and the best performance across all rows underlined.
}
  \centering
  \label{tab:tandem_adcf}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{c|l|ccc|cc|cc}
    \hline
     & \textbf{Cascade system} & 
     \multicolumn{3}{c|}{\textbf{EERs}} & 
     \multicolumn{2}{c|}{\textbf{min a-DCFs}} & \multicolumn{2}{c}{\textbf{min t-DCFs}} \\ %\cline{6-9}
     & (threshold $t$) & \textbf{SASV-EER} & \textbf{SV-EER} & \textbf{SPF-EER} & \textbf{a-DCF1} & \textbf{a-DCF2} & \textbf{t-DCF1} & \textbf{t-DCF2} \\ \hline
    \multirow{4}{*}{RawNet3 + AASIST} & ASV$\rightarrow$CM ($t_\text{asv}=0.05$) & 21.51 & 44.45 & 0.65 
    %& 0.4627 & 0.6895 & 
    & 0.1492 & 0.4316 
    & 0.0226 &  0.0644\\
     & ASV$\rightarrow$CM ($t_\text{asv}=0.5$) & 0.89 & 0.74 & 0.91 
     %& 0.0142 & 0.0189 
     & 0.1492 & 0.0506 
     & 0.0358 & 0.0918\\
     % & ASV$\rightarrow$CM ($t_\text{asv}=0.7$) & 17.13 & 17.13 & 17.13 
     %& 0.1747 & 0.2717 
     % & 0.2736 & 0.8494 
     % &  0.0524 & 0.1326\\
     % & ASV: 0.95 & 100.00 & 100.00 & 100.00 & 1.0000 & 1.0000 & 1.0000 & 1.0000 &  \\ 
     % \cline{2-9}
     & CM$\rightarrow$ASV ($t_\text{cm}=0.05$) & 1.10 & 0.69 & 1.49 
     %& 0.0191 & 0.0187 
     & 0.0240 & 0.0405 
     & N/A & N/A\\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.5$) & 0.76 & 0.71 & 0.80 
     %& 0.0153 & 0.0180 
     & 0.0180 & 0.0382 
    & N/A & N/A\\
     % & CM$\rightarrow$ASV ($t_\text{cm}=0.95$) & \textbf{0.73} & 0.80 & \underline{\textbf{0.49}} 
     %& 0.0142 & 0.0194 
     % & \textbf{0.0164} & 0.0424 
    % & N/A & N/A \\ 
    \hline
    \multirow{4}{*}{RawNet3 + AASIST-L} & ASV$\rightarrow$CM ($t_\text{asv}=0.05$) & 21.68 & 44.71 & 0.82 
    %& 0.4664 & 0.6950 
    & 0.1551 & 0.4405 
    & 0.0264 & 0.0633\\
     & ASV$\rightarrow$CM ($t_\text{asv}=0.5$) & 1.02 & 0.74 & 1.04 
     %& 0.0160 & 0.0207 
     & 0.0222 & 0.0560 
     & 0.0379 & 0.0883\\
     % & ASV$\rightarrow$CM ($t_\text{asv}=0.7$) & 17.13 & 17.13 & 17.13 
     %& 0.1757 & 0.2725 
     % & 0.2752 & 0.8519 
     % & 0.0540 & 0.1290\\
     % & ASV: 0.95 & 100 & 100 & 100.00 & 1.0000 & 1.0000 & 1.0000 & 1.0000 &  \\ 
     % \cline{2-9}

     & CM$\rightarrow$ASV ($t_\text{cm}=0.05$)& 1.58 & 0.69 & 2.24 
     %& 0.0244 & 0.0205 
     & 0.0322 & 0.0453 
     & N/A & N/A \\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.5$) & 1.02 & 0.78 & 1.30 
     %& 0.0193 & 0.0204 
     & 0.0241 & 0.0448 
     & N/A & N/A \\
     % & CM$\rightarrow$ASV ($t_\text{cm}=0.95$)& \textbf{0.82} & 0.84 & \textbf{0.73} 
     %& 0.0165 & 0.0210 
     % & \textbf{0.0198} & 0.0467 
    % & N/A & N/A \\ 
    \hline
    \iffalse
    \multirow{4}{*}{RawNet3 + LCNN} & ASV$\rightarrow$CM ($t_\text{asv}=0.05$) & 21.38 & 42.18 & 2.39 
    %& 0.4723 & 0.6919 
    & 0.1754 & 0.4541 
    & 0.0577 & 0.0995 \\
     & ASV$\rightarrow$CM ($t_\text{asv}=0.5$) & 0.89 & \textbf{0.74} & 0.91 
     %& 0.0126 & 0.0180 
     & 0.0169 & 0.0479 
     & 0.0728 & 0.1312\\
     % & ASV$\rightarrow$CM ($t_\text{asv}=0.7$) & 17.13 & 17.13 & 17.13 
     %& 0.1732 & 0.2708 
     % & 0.2713 & 0.8471 
     % & 0.0884 & 0.1704\\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.05$) & 0.63 & \textbf{0.74} & 0.52 
     %& 0.0124 & 0.0176 
     & 0.0143 & 0.0377 
     & N/A & N/A\\
     & CM$\rightarrow$ASV ($t_\text{cm}=0.5$) & 0.63 & 0.74 & 0.52 
     %& 0.0123 & 0.0176 & 
     & 0.0142 & 0.0375 
     & N/A & N/A\\
     % & CM$\rightarrow$ASV ($t_\text{cm}=0.95$) & 0.67 & 0.78 & \textbf{0.51} 
     %& 0.0126 & 0.0182 
     % & 0.0146 & 0.0392 
     % & N/A & N/A\\ 
     \fi
     \hline
    \end{tabular}
    }
\end{table*}
